Repository-Level Graph Representation Learning for Enhanced Security Patch Detection

Software vendors often silently release security patches without providing sufficient advisories (e.g., Common Vulnerabilities and Exposures) or delayed updates via resources (e.g., National Vulnerability Database). Therefore, it has become crucial to detect these security patches to ensure secure software maintenance. However, existing methods face the following challenges: (1) They primarily focus on the information within the patches themselves, overlooking the complex dependencies in the repository. (2) Security patches typically involve multiple functions and files, increasing the difficulty in well learning the representations. To alleviate the above challenges, this paper proposes a Repository-level Security Patch Detection framework named RepoSPD, which comprises three key components: 1) a repository-level graph construction, RepoCPG, which represents software patches by merging pre-patch and post-patch source code at the repository level; 2) a structure-aware patch representation, which fuses the graph and sequence branch and aims at comprehending the relationship among multiple code changes; 3) progressive learning, which facilitates the model in balancing semantic and structural information. To evaluate RepoSPD, we employ two widely-used datasets in security patch detection: SPI-DB and PatchDB. We further extend these datasets to the repository level, incorporating a total of 20,238 and 28,781 versions of repository in C/C++ programming languages, respectively, denoted as SPI-DB* and PatchDB*. We compare RepoSPD with six existing security patch detection methods and five static tools. Our experimental results demonstrate that RepoSPD outperforms the state-of-the-art baseline, with improvements of 11.90%, and 3.10% in terms of accuracy on the two datasets, respectively.

==> tables/repocpgV2.tex <==
\setlength{\algomargin}{3em} % 调整算法的左右边距
\begin{algorithm}[!tpb]

    \SetAlgoLined
    
    \footnotesize
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}

    \SetKwInOut{Initialize}{Initialize}
    \SetKwFunction{RepoCPG Construction}{RepoCPG Construction}
    \SetKwProg{Fn}{Function}{:}{}
    \Input{Pre\_code: $Code\_pre$, Post\_code: $Code\_post$, Repo\_Function: $Repo\_func$ }
    \Output{RepoCPG, $RepoCPG$}
    % \Initialize{Initialize an action list $ac\_list$ }
    \Fn{RepoCPG Construction}{
    // Generating the Pre-Patch and Post-Patch CPGs
    
    $Pre\_CPG(N\_pre, E\_pre) \leftarrow Code\_pre$ 
    
    $Post\_CPG(N\_post, E\_post) \leftarrow Code\_post$

    // Fuse the Pre\_CPG and Post\_CPG to obtain the MergeCPG.
    
    \For{$v \leftarrow N\_pre, N\_post, E\_pre, E\_post$}
    {
    \eIf{$v \in V\_pre \ \textbf{and} \ v \in V\_post$}{
        $v.\text{type} \gets \text{fuse}$\;
    }{
        \If{$v \in V\_pre$}{
            $v.\text{type} \gets \text{pre}$\;
        }
        
            \If{$v \in V\_post$}{
                $v.\text{type} \gets \text{post}$\;
            }
        
    }
    Construct $MergeCPG$
    
    }

    // Integrating the repository-level dependency.
    
    \If{$node$.type $\in$ Call\_graph}
        {
        // Adopt static tool to extract $Function\_name$ in the repository

        \If{$Function\_name$ $\in$ $Repo\_func$}
        {
            $Call\_func$ $\leftarrow$ $Repo\_func[i]$
            
            // Construct the $Call\_CPG$  of $Call\_func$ 
            
            $Call\_CPG$ $\leftarrow$ $Call\_func$ 
            
            // Find the $root\_node$ of $Call\_CPG$
            
            Add Edge ($node, root\_node$) and sign the $root\_node$ as $R$

            // Update MergeCPG
            
            $RepoCPG(N, E, R)$ $\leftarrow$ $MergeCPG$
            
        }
        
        
        }
        
    // Slicing code changes in repository-level.
    
    \If{$R$$\in$ Code Change}
        {// Adding Slicing
        
        Slice  $RepoCPG(N, E, R)$
        
        // Removing Slicing

        Slice  $RepoCPG(N, E, R)$
        }
    \Return {$RepoCPG(N, E, R)$}
    }
    
    
    
\caption{\graph Construction}
\label{algorithm1}

\end{algorithm}
